GroundCascade: Selective Second Opinions for GUI Grounding

Graphical user interface (GUI) grounding maps a screenshot and a natural-language instruction to the screen location where an agent should act. Zoomed views can reveal small targets but may lose the context needed to identify them. We introduce GroundCascade, a training-free controller that uses agreement between a grounder's full-screen and zoomed predictions to decide when to consult a complementary model. It selects between zoomed predictions while preserving corroborated full-screen locations. An optional Finalizer predicts from an unmarked joint crop when disagreement remains (Full); omitting it yields the two-stage Selective variant. GroundCascade reaches 85.33% on ScreenSpot-Pro with Indeed-UI-32B/8B/32B and 88.43% on the visible-target OSWorld-G-Refined subset with Qwen3.6-27B/3.8-27B/3.8-27B, gains of 2.66 and 2.35 percentage points over the stronger standalone two-pass grounder. On UI-Vision, GroundCascade reaches 72.20% category-balanced accuracy, with Selective slightly higher at 72.28%. Across these three evaluations, GroundCascade in Full mode uses 2.42-2.73 calls per request, 31-39% fewer than unconditionally acquiring both models' two-pass predictions. At matched second-model call budgets, selective acquisition gains 1.52-2.56 points over standalone Two-pass, compared with 0.22-0.69 points from stratified random acquisition. GroundCascade leads the official ScreenSpot-Pro leaderboard and exceeds reported GUI-specialist comparisons on OSWorld-G-Refined and UI-Vision, subject to differences in external evaluation protocols.

==> figures/qualitative_panels.tex <==
\colorlet{gcg}{gcG}\colorlet{gcr}{gcR}\colorlet{gcf}{gcF}\colorlet{gctarget}{gcTarget}% figures/gcpalette.tex
% Both Context and Detail markers use one radius and one halo width.
\def\GCQualRadius{3.0pt}
\def\GCQualOutlineWidth{1.1pt}
\def\GCQualHaloWidth{2.5pt}
\tikzset{gcqualhalo/.style={draw=white,line width=\GCQualHaloWidth}}

\newcommand{\GCQualCircle}[4]{%
  \path[gcqualhalo] (#1,#2) circle (\GCQualRadius);
  \draw[draw=#3,fill=#4,line width=\GCQualOutlineWidth]
    (#1,#2) circle (\GCQualRadius);
}
\newcommand{\GCQualStar}[2]{%
  \node[font=\large,text=gcf,inner sep=0pt] at (#1,#2) {%
    \pdfliteral direct {q 1 Tr 2 w 1 1 1 RG}% stroke-only white glyph outline
    $\star$%
    \pdfliteral direct {Q}%
  };
  \node[font=\large,text=gcf,inner sep=0pt] at (#1,#2) {$\star$};
}

\newcommand{\GCAndroidPanel}{%
\begin{tikzpicture}[x=1pt,y=-1pt,inner sep=0pt,outer sep=0pt]
\path[use as bounding box] (0,0) rectangle (243,121.5);
\node[anchor=north west] at (0,0) {\includegraphics[width=243pt]{figures/qualitative_android17.png}};
\begin{scope}[shift={(0,-37)}]
\draw[draw=gctarget,line width=1.3pt] (63.18,95.9275) rectangle (78.975,114.1525);
\GCQualCircle{75.9375}{103.825}{gcg}{white}
\GCQualCircle{49.2075}{103.825}{gcg}{gcg}
\GCQualCircle{155.52}{126.3025}{gcr}{white}
\GCQualCircle{154.305}{128.125}{gcr}{gcr}
\GCQualStar{68.04}{104.4325}
\end{scope}
\end{tikzpicture}%
}

\newcommand{\GCVSCodePanel}{%
\begin{tikzpicture}[x=1pt,y=-1pt,inner sep=0pt,outer sep=0pt]
\path[use as bounding box] (0,0) rectangle (243,121.5);
\node[anchor=north west] at (0,0) {\includegraphics[width=243pt]{figures/qualitative_vscode15.png}};
\begin{scope}[shift={(-261,-37)}]
\draw[draw=gctarget,line width=1.3pt] (462.0825,119.0125) rectangle (477.8775,133.5925);
\GCQualCircle{468.1575}{66.16}{gcg}{white}
\GCQualCircle{275.58}{97.1425}{gcg}{gcg}
\GCQualStar{467.55}{126.3025}
\end{scope}
\end{tikzpicture}%
}

